The low density and magnetization of a massive galaxy halo exposed by a fast radio burst

Present-day galaxies are surrounded by cool and enriched halo gas extending to hundreds of kiloparsecs. This halo gas is thought to be the dominant reservoir of material available to fuel future star formation, but direct constraints on its mass and physical properties have been difficult to obtain. We report the detection of a fast radio burst (FRB 181112) with arcsecond precision, which passes through the halo of a foreground galaxy. Analysis of the burst shows the halo gas has low net magnetization and turbulence. Our results imply predominantly diffuse gas in massive galactic halos, even those hosting active supermassive black holes, contrary to some previous results.

==> ASKAPfieldsrcs_table.tex <==
\begin{table*}
\centering
\caption{JMFIT positions and flux densities of the 3 brightest ASKAP field sources \label{tab:ASKAPsrcs}}
\begin{minipage}{270mm} 
\begin{tabular}{*{7}{c}}
\hline 
Source & R.A. & R.A.$_{\textrm{err}}$ & Dec. & Dec.$_{\textrm{err}}$ & S & S$_{\textrm{err}}$ \\ 
& (J2000) & (mas) & (J2000) & (mas) & (mJy) & (mJy beam$^{-1}$)
\\ 
\hline 
SUMSS 2151-5316 & 21:51:55.367 & 2148.148 & $-$53:16:47.51 & 1350.0 & 40.877 & 3.76 \\ 
SUMSS 2150-5255 & 21:50:37.155 & 2120.956 & $-$52:55:40.02 & 1440.0 & 33.905 & 3.79 \\ 
SUMSS 2156-5329 & 21:56:06.321 & 2936.709 & $-$53:29:11.20 & 1790.0 & 29.539 & 3.74 \\ 
\hline 
\end{tabular} 
\end{minipage} 
\end{table*} 

==> ATCAcaltable.tex <==
\begin{table*}
\centering
\caption{Phase calibrators used for ATCA observation and the position of the SUMSS 2151-5316 derived using these calibrators. \label{tab:ATCAcal}}
\begin{minipage}{270mm} 
\begin{tabular}{ccc}
\hline 
Source & R.A.  & Dec.  
\\
& (J2000)  & (J2000) 
\\ 
\hline 

\textbf{Calibrators used}   & & \\
2117-642 & 21:21:55.0217  & $-$64:04:30.042  \\ 
%2134-470 & 21:38:01.07 & 83.3 & $-$46:46:40.51 & 38.0 \\ 
2215-508 & 22:18:19.02  & $-$50:38:41.73  \\
\\
\textbf{FRB~181112 field source}  & & \\
SUMSS 2151-5316$_{2117-642}$ & 21:51:55.30
 & $-$53:16:46.565
 \\
SUMSS 2151-5316$_{2215-508}$ & 21:51:55.29
 & $-$53:16:47.09 
  \\
\hline
\end{tabular}
\end{minipage}
\end{table*}

==> tab_fg.tex <==
\begin{table}
\centering
\caption{Results from CIGALE and nebular line analysis of the foreground galaxy\label{tab:host}}
\begin{minipage}{270mm} 
\begin{tabular}{ccccc}
\hline 
Package & Parameter & Value & Uncertainty & Unit 
\\ 
\hline 
CIGALE & AGN Fraction & 0.1 & 0.2 & \\ 
CIGALE & Metallicity & 0.017 & 0.016 & \\ 
CIGALE & $u-r$ & 2.3 & 0.1 & rest-frame \\ 
CIGALE & $M_r$ & -21.98 & 0.05 & rest-frame \\ 
pPXF & $E(B-V)$ & 0.07 & 0.20 & mag \\ 
pPXF & [N{\sc ii}]/H$\alpha$ & 0.28 & 0.03 & log10 \\ 
pPXF & [O{\sc iii}]/H$\beta$ & 1.10 & 0.05 & log10 \\ 
\hline 
\end{tabular} 
\end{minipage} 
\end{table} 


==> tab_host.tex <==
\begin{table}
\centering
\caption{\hgname\ Results from CIGALE and nebular line analysis of the host galaxy\label{tab:host}}
\begin{minipage}{270mm} 
\begin{tabular}{ccccc}
\hline 
Package & Parameter & Value & Uncertainty & Unit 
\\ 
\hline 
CIGALE & Stellar Mass & 0.26 & 0.1& $10^{10} M_\odot$ \\ 
CIGALE & AGN Fraction & 0.0 & 0.0 & \\ 
CIGALE & $u-r$ & 1.2 & 0.2 & rest-frame \\ 
CIGALE & $M_r$ & -20.34 & 0.07 & rest-frame \\ 
CIGALE & SFR & 0.4 & 0.6 & $M_\odot \, \rm yr^{-1}$ \\ 
CIGALE & $E(B-V)$ & 0.15 & 0.08 & mag \\ 
pPXF & SFR$_\beta$ & 0.57 & 0.17 &  $M_\odot \, \rm yr^{-1}$ \\ 
\hline 
\end{tabular} 
\end{minipage} 
\end{table} 


==> tab_line_fluxes.tex <==
\begin{table}
\centering
\caption{Galaxy Nebular Emission\label{tab:lines}}
\begin{minipage}{270mm} 
\begin{tabular}{cccccc}
\hline 
Galaxy & Line & Flux & Flux Uncertainty & Luminosity$^a$ & Lum. Error \\ 
&& ($10^{-17}$ erg/s/cm$^2$) & ($10^{-17}$ erg/s/cm$^2$) 
& ($10^{40}$ erg/s) & ($10^{40}$ erg/s) 
\\ 
\hline 
Host& H $\alpha$ & 6.4 & 0.8 & 5.8 & 0.7\\ 
Host& H $\beta$ & 2.9 & 0.2 & 2.6 & 0.2\\ 
Host& H $\gamma$ & 0.7 & 0.2 & 0.6 & 0.2\\ 
Host& {[NII]  6584} & 4.9 & 1.0 & 4.4 & 0.9\\ 
Host& {[OIII]  5007} & 5.4 & 0.3 & 4.9 & 0.3\\ 
Foreground& H $\alpha$ & 5.5 & 0.3 & 3.4 & 0.2\\ 
Foreground& H $\beta$ & 1.8 & 0.2 & 1.2 & 0.1\\ 
Foreground& {[NII]  6584} & 10.5 & 0.5 & 6.5 & 0.3\\ 
Foreground& {[OIII]  5007} & 23.0 & 0.3 & 15.5 & 0.2\\ 
\hline 
\end{tabular} 
\end{minipage} 
{$^a$} Extinction-corrected 
\end{table} 


==> tab_photom.tex <==
\begin{table}
\centering
\caption{Galaxy Photometry\label{tab:photom}}
\begin{minipage}{270mm} 
\begin{tabular}{ccccc}
\hline 
Galaxy & Survey & Filter & Value & Uncertainty$^a$
\\ 
\hline 
Host & DES-DR1 & g & 22.71 & 0.09 \\ 
Host & DES-DR1 & r & 21.73 & 0.05 \\ 
Host & DES-DR1 & i & 21.49 & 0.06 \\ 
Host & DES-DR1 & z & 21.45 & 0.11 \\ 
Host & DES-DR1 & Y & 21.07 & 0.17 \\ 
Host & VLT & g & 22.57 & 0.04 \\ 
Host & VLT & I & 21.51 & 0.04 \\ 
\hline 
Foreground & DES-DR1 & g & 21.42 & 0.03 \\ 
Foreground & DES-DR1 & r & 19.90 & 0.01 \\ 
Foreground & DES-DR1 & i & 19.34 & 0.01 \\ 
Foreground & DES-DR1 & z & 19.03 & 0.01 \\ 
Foreground & DES-DR1 & Y & 18.86 & 0.02 \\ 
Foreground & VLT & g & 21.20 & 0.04 \\ 
Foreground & VLT & I & 19.20 & 0.02 \\ 
Foreground & WISE & W1 & 15.53 & 0.04 \\ 
Foreground & WISE & W2 & 14.89 & 0.06 \\ 
Foreground & WISE & W3 & 12.28 & -999.00 \\ 
Foreground & WISE & W4 & 8.59 & -999.00 \\ 
\hline 
\end{tabular} 
\end{minipage} 
{$^a$}Uncertainty $\le 0$ indicates an upper limit.\\ 
\end{table} 


==> tab_sersic.tex <==
\begin{table}
\centering
\caption{GALFIT S\'{e}rsic profile fits\label{tab:sersic}}
\begin{minipage}{270mm} 
\begin{tabular}{ccccc}
\hline 
Galaxy & S\'{e}rsic index & Index fit error & Half-light radius& Half-light radius error \\ 
 & & & (arcsec) & (arcsec)\\ 
\\ 
\hline 
HG181112 & 1.9 & 0.4 & 0.64 & 0.04\\ 
FG181112\_13\_5 & 2.48 & 0.08 & 0.760 & 0.008\\ 
\hline 
\end{tabular} 
\end{minipage}
\end{table} 

==> tab_summary.tex <==
\begin{table*}
\centering
Table \tabsumm: \caption {{\bf Properties of FRB~181112, its host, and the foreground galaxy \fgname.} \\ 
See \cite{supp} for details on the measurements and the main text for the derived constraints on the 
magnetic field, density, and filling factor.}\begin{tabular}{|l r|}
\hline 
FRB & \\ 
\hline 
Right Ascension (J2000) & $327.34846 \pm 0.00015$ \, deg \\ 
Declination (J2000) & $-52.97093 \pm 0.00004$ \, deg \\ 
Dispersion measure (\dmfrb) & $589.27 \pm 0.03$\, pc cm$^{-3}$ \\ 
Rotation measure (RM) & $10.9 \pm 0.9$\, rad m$^{-2}$ \\ 
Pulse width & $< 40 \, \upmu$s \\ 
\hline 
Host Galaxy & \\ 
\hline 
Redshift & $\zfrb \pm 0.00015$ \\ 
Stellar Mass & $2.6 \pm 1.1$ $\, \times 10^{9} M_\odot$  \\ 
Star formation rate & $0.6$\, \msun \, yr$^{-1}$\\ 
\hline 
Foreground galaxy \fgname & \\ 
\hline 
Redshift & $0.36738 \pm 0.00007$ \\ 
Impact parameter to the FRB sightline ($\mrperp$) & $\rperpv \pm 3$ \, kpc \\ 
Stellar Mass & $4.9 \pm 3.2\, \times 10^{10} M_\odot$ \\ 
Star formation rate & $<0.3\, M_\odot \, \rm yr^{-1}$\\ 
Coherent magnetic field parallel to the line of sight & $B_\parallel <0.8 {\rm \upmu G} \, (n_e/10^{-3} \rm cm^{-3})$ \\ 
Density constraint for hot, diffuse gas ($f_V \sim 1$) & $n_e < 2 \times 10^{-3} \rm cm^{-3}$ \\ 
Filling factor constraint for cool, clumpy gas & $f_V < 10^{-4}$ \\ 
\hline 
\end{tabular} 
\end{table*} 

